Augmented-Reality Enabled Crop Monitoring with Robot Assistance

The integration of augmented reality (AR), extended reality (XR), and virtual reality (VR) technologies in agriculture has shown significant promise in enhancing various agricultural practices. Mobile robots have also been adopted as assessment tools in precision agriculture, improving economic efficiency and productivity, and minimizing undesired effects such as weeds and pests. Despite considerable work on both fronts, the combination of a versatile User Interface (UI) provided by an AR headset with the integration and direct interaction and control of a mobile field robot has not yet been fully explored or standardized. This work aims to address this gap by providing real-time data input and control output of a mobile robot for precision agriculture through a virtual environment enabled by an AR headset interface. The system leverages open-source computational tools and off-the-shelf hardware for effective integration. Distinctive case studies are presented where growers or technicians can interact with a legged robot via an AR headset and a UI. Users can teleoperate the robot to gather information in an area of interest, request real-time graphed status of an area, or have the robot autonomously navigate to selected areas for measurement updates. The proposed system utilizes a custom local navigation method with a fixed holographic coordinate system in combination with QR codes. This step toward fusing AR and robotics in agriculture aims to provide practical solutions for real-time data management and control enabled by human-robot interaction. The implementation can be extended to various robot applications in agriculture and beyond, promoting a unified framework for on-demand and autonomous robot operation in the field.

==> leftover.tex <==
\section{Technical Analysis}
\label{sec:methods}
\todo{Make leftover tex and add all equations there.}
We can write our pneumatic system considering input $u(t)$ as the PWM signal to the pneumatic controller to actuate the pumps (and therefore regulate the airflow), and perturbation $\rho(t)$ (assumed to be unknown but uniformly bounded) to the input $u(t)$ as
%
\begin{equation}
    \ddot{\theta}(t) = u(t) + \rho(t)
    \label{eq:each}
\end{equation}
%
which is a second-order system with disturbance $\rho$. Letting a finite $r$-th order polynomial bound the disturbance, i.e.
%
\begin{equation}
    \rho(t)= \sum_{i=0}^{r}\alpha_it^i\enspace,
\end{equation}
%
the error dynamics can then be given by
\begin{equation}
    \ddot{e} = u +  \sum_{i=0}^{r}\alpha_it^i
    \label{eq:err1}
\end{equation}
%
which will require the controller feedback to grow the input signal $u(t)$ in a similar polynomial rate. By integration,
%
\begin{equation}
    \dot{e} = \dot{e}(0) + \int u + \int \sum_{i=0}^{r}\alpha_it^i
    \label{eq:integr}
\end{equation}

Integrating~\eqref{eq:integr} again, it can be seen that $r+2$ different integral gains are necessary to manipulate all terms in it~\cite{luviano2008chaotic}. With a feedback controller of the form
%
\begin{equation}
\begin{aligned}
    u = -k_{r+3} \int u -k_{r+2} e -k_{r+1} \int e -k_{r} \int\int e -...\\- k_1\int^{r+1}e - k_0\int^{r+2}e
    \end{aligned}
    \label{eq:ll}
\end{equation}
%
or in its equivalent Laplace form,
%
\begin{equation}
    u(s) =e\left(k_{r+2} + \frac{k_{r+1}}{s} +...+ \frac{k_1}{s^{r+1}} + \frac{k_0}{s^{r+2}} \right) -\frac{k_{r+3}}{s}u\enspace,
    \label{eq:ccon}
\end{equation}
%
the closed-loop error dynamics system then becomes
%
\begin{equation}
\begin{aligned}
    \ddot{e} + k_{r-3} \dot{e} + k_{r-2} e + k_{r-1} \int e + k_{r} \int\int e +...\\+ k_1\int^{r+1}e + k_0\int^{r+2}e =
    k_{r+3}\sum_{i=0}^{r}\alpha_it^i + k_{r+3}e(0)
    \end{aligned}
    \label{eq:eh}
\end{equation}
%
The $r+2$ derivative of~\eqref{eq:eh} leads to
%
\begin{equation}
\begin{aligned}
    e^{r+4} + k_{r+3}e^{r+3} + k_{r+2}e^{r+2} + ... + k_{m-1}e^{r-1} \\ + ...+k_1\dot{e} + k_0e =0\enspace,
\end{aligned}
\end{equation}
%
with characteristic equation
%
\begin{equation}
    P(s) = s^{r+4} + k_{r+3}s^{r+3} + k_{r+2}s^{r+2} + ... +k_1s+k_0\enspace.
\label{eq:polcal}
\end{equation}

Selecting $p(s)$ real roots to be negative will result in the error tracking problem converging asymptotically to zero, which is desirable in trajectory tracking. The controller can be thus described as a lead compensator based on~\eqref{eq:ccon}, i.e.

\begin{equation}
\begin{aligned}
K_{GPI}(s) &= \left(\frac{k_{r+2}s^{r+2}+k_{r+1}s^{r+1}+...+k_1s + k_0}{s^{r+1}(s+k_{r+3})} \right)\enspace,\\
    u &= - K_{GPI}(s)e\enspace.
    \end{aligned}
    \label{eq:controlad}
\end{equation}
%
For a desired reference trajectory $\theta_d(t)$, the tracking and input errors are $e = \theta - \theta_d(t)$ and $e_u = u - u_d(t)$, respectively. Then,  
%
\begin{equation}
    u(t) = u_d(t) - K_{GPI}(\theta-\theta_d(t))\enspace,
    \label{eq:ccon1}
\end{equation}
%
where $u_d(t)$ is determined according to the unperturbed system ($\rho(t)=0$) in~\eqref{eq:each}. Treating each DoF of the wearable device as a spring-mass-damper system, the transfer function which relates the PWM \% of the pneumatic actuator and angle $\theta_i$ of the respective supported segment of the arm, attains the form
%
\begin{equation}
    G_i(s) = \frac{\gamma_{0_i}}{s^2 + \gamma_{1_i} s + \gamma_{2_i}}\enspace.
    \label{eq:mass}
\end{equation}
 
For a constant value perturbation at $t=\tau$ we get
%
\begin{equation}
\ddot{\theta}(t) = u(t) + \rho1(t-\tau) 
\end{equation}
%
and with $r=0$, \eqref{eq:controlad} becomes
%
\begin{equation}
    K_{GPI}(s) = \frac{k_2s^2+k_1s+k_0}{s(s+k_3)}\enspace.
\end{equation}

Rewriting~\eqref{eq:ccon1}, and dividing the controller constant values by $1/\gamma_{0_i}$ yields 
%
\begin{equation}
        u(t) = u_d(t) - \left(\frac{1}{\gamma_{0_i}}\frac{k_2s^2+k_1s+k_0}{s(s+k_3)}\right)e
        \label{eq:imple}
\end{equation}
%
since $e(s)=G_i(s)e_u(s)$ relates the input and output errors. Combining with~\eqref{eq:mass}, we get
%
\begin{equation}
    \left[1+\left( \frac{1}{s^2 + \gamma_{1_i} s + \gamma_{2_i}} \right) \left( \frac{k_2s^2+k_1s+k_0}{s(s+k_3)}\right)\right]e=0
    \label{eq:both}
\end{equation}
%
leading to the characteristic equation 
\begin{equation}
\begin{aligned}
    s^4 + (k_3+\gamma_{1_i})s^3 + (k_2 + k_3\gamma_{1_i}+\gamma_{2_i})s^2 +\\ (k_3\gamma_{2_i}+k_1)s + k_0 = 0\enspace.
    \label{eq:1}
    \end{aligned}
\end{equation}

The controller gains $k_i$ can be determined by factoring the Hurwitz polynomial (therefore having poles located in the half left complex plane), i.e.
%
\begin{equation}
    (s^2 + 2\xi w_n^2+w_n^2)^2 = 0\enspace,
    \label{eq:2}
\end{equation}
%
which yields
\begin{equation}
    \begin{aligned}
        &k_0 = w_n^4\enspace, \\
        &k_1 = 4w_n^3\xi - \gamma_{2_i}(4\xi w_n-\gamma_{1_i})\enspace,\\
        &k_2 = 2w_n^2 + 4\xi^2w_n^2 - \gamma_{1_i}(4\xi w_n - \gamma_{1_i}) - \gamma_{2_i}\enspace,\\
        &k_3 = 4\xi w_n - \gamma_{1_i}\enspace.
    \end{aligned}
    \label{eq:third}
\end{equation}

Therefore, our controller can be determined with parameters from~\eqref{eq:third}. The controller design parameters are the values $\xi_i$ and $w_{n_i}$, both positive quantities. From~\eqref{eq:imple} we can implement the controller as 
%
\begin{equation}
\begin{aligned}
    u = u_d - k_3(\dot{\theta_{int}}-\dot{\theta_d}) + \\ \frac{1}{\gamma_{0_i}}\left[ -k_2(e-e_0) - k_1\int_t e dt  - k_0\iint_t e dt \right] \enspace,
    \end{aligned}
    \label{eq:controlad}
\end{equation}
%
where $u$ is the output, $\theta_{int}$ is the integral reconstruction \cite{romero2014algebraic,blanco2022robust} of the input $u$, as in \eqref{eq:integr} substituting $r=0$
%
\begin{equation}
\begin{aligned}
        \theta_{int} = \int_{0}^{t} u dt \\
        \dot{\theta} = \theta_{int} -\dot{\theta_0}
            \label{eq:ust}
\end{aligned}
\end{equation}
%
and the value $u_d$ is given by~\cite{sira2007fast}, 
%
\begin{equation}
    u_d = \frac{1}{\gamma_{0_i}}[\ddot{\theta_d} + \gamma_{1_i}\dot{\theta_d}+\gamma_{2_i}\theta_d]\enspace.
\end{equation}

For both~\eqref{eq:controlad} and~\eqref{eq:ust}, the integral values are numerically estimated by the trapezoidal rule. 


%The previous analysis considered a ramp type disturbance $\rho(t)$. To introduce robustness to the controller for the 3DOF device, we can assume a polynomial type disturbance:

%\begin{equation}
%    \rho(t) = \alpha_1t^4 + \alpha_2t^5 + \alpha_3t^2 + \alpha_4t+\alpha_5
%    \label{eq:distur}
%\end{equation}

%Looking at eq. \ref{eq:controlad}, with $r=4$, this will lead to the %controller

%\begin{equation}
%\begin{aligned}
%K_{GPI}(s) = \left(\frac{k_6s^6+k_5s^5+...+k_1s + k_0}{s^5(s+k_7)} \right)\\
%    u = - K_{GPI}(s)e 
%    \end{aligned}
%    \label{eq:controladd}
%\end{equation}


%from eq. \ref{eq:mass} and similarly to as in eq.\ref{eq:both}

%\begin{equation}
%    \left[1+\left( \frac{1}{s^2 + \gamma_{1_i} s + \gamma_{2_i}} \right) \left(\frac{k_6s^6+k_5s^5+...+k_1s + k_0}{s^5(s+k_7)} \right)\right]e=0
%\end{equation}

%leading to:

%\begin{equation}
%    \begin{aligned}
%    s^8 + (\gamma_{1_i} + k_7)s^7+ (\gamma_{1_i}k_7 + \gamma_{2_i}+k_6)s^6 
%    + (\gamma_{2_i} k_7 + k_5)s^5 \\ + k_4 s^4 + k_3 s^3 + k_2 s^2
%    + k_1 s + k_0
%    \end{aligned}
%    \label{eq:poll}
%\end{equation}

%\noindent The tracking error polynomial characteristic becomes as per eq. \ref{eq:polcal}:

%\begin{equation}
%    (s^2 + 2\xi_iw_{n_i}s + w_{n_i}^2)^4 = 0
%    \label{eq:dess}
%\end{equation}

%\noindent which leads to:
%s^8 + 8 c s^7 w + (4  w^2 + 24 c^2 w^2) s^6 + (24 c w^3 + + 32 c^3  w^3)s^5 +
%(16 c^4 w^4 + 48 c^2 w^4 +6 w^4 )s^4 + (24 c w^5 + 32 c^3 w^5) s^3  + (4 w^6 + 24 c^2 w^6) s^2 + 8 c w^7 s + w^8

%\begin{equation}
%    \begin{aligned}
%s^8 + 8 \xi_i  w_{n_i} s^7 + (4  w_{n_i}^2 + 24 \xi_i^2 w_{n_i}^2) s^6 + (24 \xi_i w_{n_i}^3 + 32 \xi_i^3  w_{n_i}^3)s^5 +\\
%(16 \xi_i^4 w_{n_i}^4 + 48 \xi_i^2 w_{n_i}^4 +6 w_{n_i}^4 )s^4 + (24 \xi_i w_{n_i}^5 + 32 \xi_i^3 w_{n_i}^5) s^3 \\ + (4 w_{n_i}^6 + 24 \xi_i^2 w_{n_i}^6) s^2 + 8 \xi_i w_{n_i}^7 s + w_{n_i}^8
 %   \end{aligned}
 %   \label{eq:eit}
%\end{equation}


%\noindent and comparing eqs.\ref{eq:poll} and \ref{eq:eit} , we have that:
%\begin{equation}
%    \begin{aligned}
%        &k_0 = w_{n_i}^8 \\
%        &k_1 =  8 \xi_i w_{n_i}^7\\
%        &k_2 = 4 w_{n_i}^6 + 24 \xi_i^2 w_{n_i}^6  \\
%        &k_3 = 24 \xi_i w_{n_i}^5 + 32 \xi_i^3 w_{n_i}^5  \\
%        &k_4 = 16 \xi_i^4 w_{n_i}^4 + 48 \xi_i^2 w_{n_i}^4 +6 w_{n_i}^4   \\
%        &k_5 =  24 \xi_i w_{n_i}^3 + 32 \xi_i^3  w_{n_i}^3 - \gamma_{2_i} (8 \xi_i  w_{n_i}  -  \gamma_{1_i}) \\
%        &k_6 =  4  w_{n_i}^2 + 24 \xi_i^2 w_{n_i}^2 - (\gamma_{1_i}(8 \xi_i  w_{n_i}  -  \gamma_{1_i}) + \gamma_{2_i})  \\
%        &k_7 = 8 \xi_i  w_{n_i}  -  \gamma_{1_i}
%    \end{aligned}
%    \label{eq:par}
%\end{equation}

%Therefore our controller can be determined with parameters from \ref{eq:par}. For both eqs. \ref{eq:third} and \ref{eq:par}, the controller design parameteres are the values $\xi_i$ and $w_{n_i}$, both positive quantities.
